Data Games: A Game-Theoretic Approach to Swarm Robotic Data Collection

Fleets of networked autonomous vehicles (AVs) collect terabytes of sensory data, which is often transmitted to central servers (the ''cloud'') for training machine learning (ML) models. Ideally, these fleets should upload all their data, especially from rare operating contexts, in order to train robust ML models. However, this is infeasible due to prohibitive network bandwidth and data labeling costs. Instead, we propose a cooperative data sampling strategy where geo-distributed AVs collaborate to collect a diverse ML training dataset in the cloud. Since the AVs have a shared objective but minimal information about each other's local data distribution and perception model, we can naturally cast cooperative data collection as an $N$-player mathematical game. We show that our cooperative sampling strategy uses minimal information to converge to a centralized oracle policy with complete information about all AVs. Moreover, we theoretically characterize the performance benefits of our game-theoretic strategy compared to greedy sampling. Finally, we experimentally demonstrate that our method outperforms standard benchmarks by up to $21.9\%$ on 4 perception datasets, including for autonomous driving in adverse weather conditions. Crucially, our experimental results on real-world datasets closely align with our theoretical guarantees.

==> fig_latex/digital_twin.tex <==
\begin{figure}[t]
    \begin{minipage}[c]{0.5\textwidth}
        \includegraphics[width=\columnwidth]{pics/Expeditions_Robotics.pdf}
      \end{minipage}\hfill
      \begin{minipage}[c]{0.5\textwidth}
        \includegraphics[width=\columnwidth]{pics/Expeditions_Digital_Twin.pdf}
    \end{minipage} 
\end{figure}


==> fig_latex/hardware_times.tex <==
\newcommand{\putsmallfig}[1]{\includegraphics[width=3cm]{#1}}

\begin{table*}
        \centering
        \begin{tabular}{|c|c |c| c|}
        \hline
            \small \textbf{Robot Id}&
            \small \textbf{Inference Time} & 
            \small\textbf{Policy Computation Time} & 
            \small\textbf{Communication Time} \\
            \hline
            \hline
            
            \small \textbf{Robot 1} &
            $7.45 \pm 0.10 \mathrm{ms}$ &
            $51.9 \pm 4.86 \mathrm{ms}$ &
            \multirow{3}{4em}{$17.0 \pm 4.04 \mathrm{ms}$} \\
            \cline{1-3}
            
            \small \textbf{Robot 2} &
            $7.48 \pm 0.06 \mathrm{ms}$ &
            $53.6 \pm 3.87 \mathrm{ms}$ &
            \\
            \cline{1-3}
            \small \textbf{Robot 3} &
            $7.58 \pm 0.13 \mathrm{ms}$ &
            $51.8 \pm 3.20 \mathrm{ms}$ &
            \\
            \hline
            
        \end{tabular}
        \caption{\rebuttal{\small{\textbf{ Small Hardware Deployment on 3 Nvidia Jetson Nano Embedded GPUs.}
        We confirmed that it is scalable to run a vision model, compute an action (rate to upload data) using a convex solver, and run our \Interactive~ policy on a low-power embedded GPU commonly used in robotics. We did not have access to a large fleet of robots, so simply used 3 devices.}}}
        \label{fig:hardware_times}
    \end{table*}
    


==> sections/algo.tex <==

\Interactive: Algorithm \ref{alg:train} shows the complete procedure for calculating the proposed sampling strategy for each robot at the end of the round $r$. The algorithm calculates action, $\action{r}{i}$, for each robot after all robots have collected their local datasets $\devicedataset{r}{i}$. The algorithm takes the target dataset $\datasettarget$ as inputs (line \ref{ln:inputs}). 
We initialize each robot's actions, $\action{r}{i}$ in lines \ref{ln:for1_loop} - \ref{ln:for1_loop_end}, using the \Greedy \space action policy (\ref{eq:indvopt}) because the robots have no information about other robot's collected datasets (line \ref{ln:init_actions}) and can only take greedy actions.
In lines \ref{ln:share_init_actions} - \ref{ln:for2_loop_end}, we calculate optimal actions for each robot using our proposed \Interactive \space action policy. Each robot is trying to minimize the convex distance, $\kl{r}$, between the current cloud dataset and the target dataset, $\datasettarget$, by choosing an action $\action{r}{i}$ for itself.
The key intuition behind our \Interactive \space action policy is that each robot will be able to contribute better (i.e. help in reducing the cloud dataset distance) if it is aware of other robot's actions.  We start by sharing the initial actions for each robot (calculated in line \ref{ln:init_actions}) with all robots (line \ref{ln:share_init_actions}). Then we iterate through each robot (lines \ref{ln:for2_loop} - \ref{ln:for2_loop_end}) and calculate its best action, $\action{r}{i}$, using the optimization program \ref{eq:interactiveopt} while considering the shared best action of other robots, $\action{r}{j}; j \neq i = 0, \ldots, \ndevice$,  (line \ref{ln:interactive_opt}). The optimization program \ref{eq:interactiveopt}, is very similar to that of \Oracle \space policy (Eq. \ref{eq:oracleopt}), with the only difference being the calculation of the cloud dataset at round $r +1$, Eq. \ref{eq:dataset_inter}.
Optimization program \ref{eq:interactiveopt} uses actions of other robots to calculate robot $i$'s best action. In line \ref{ln:share_calc_actions}, each robot shares its optimal action calculated using opt. program (\ref{eq:interactiveopt}) with other robots. This repeats procedure until our system reaches the Nash equilibrium (i.e. a fixed point, where no robot would change its action).  Finally in lines \ref{ln:for3_loop} - \ref{ln:for3_loop_end}, after convergence, we share each robot's final calculated action $\action{r}{i}$ with the cloud (line \ref{ln:share_cache}). Reader should note that \Interactive \space policy optimization program \ref{eq:interactiveopt} has a convex objective with linear constraints. Therefore, it is guaranteed to converge to an optimal solution (see Thm. 1 \ref{theorem:converge_eventually}).


==> sections/checklist.tex <==
% For the paper checklist
\newcommand{\answerYes}[1]{{\color{blue}{[Yes]#1}}}
\newcommand{\answerNo}[1]{{\color{red}{[No]#1}}}
\newcommand{\answerNA}[1]{{\color{red}{[N/A]#1}}}
\newcommand{\answerTODO}[1]{{\color{red}{\bf[TODO]}}}

\noindent \textbf{Paper Submission Checklist}

\noindent \textbf{Student Name: Shubhankar Agarwal} \newline
\noindent \textbf{Peer Reviewer Name: Po-han and Oguzhan}  \newline
\noindent \textbf{Paper Title: A Game Theoretic Approach to Cooperative Data-Offloading in Networked IoT Devices} \newline
\noindent \textbf{Date: \today} \newline

\begin{enumerate}
    \item Did you spell check and grammar check the full document, using Grammarly if needed?
    \answerYes{}
    \item Did you organize the LaTeX files according to the sample paper guide, including naming the file appropriately, organizing sections etc.? \answerYes{}
  \item Did you make sure all plots are legible, in at least 20 point font, and ideally use the lab plotting tools/guidelines? \answerYes{}
  \item Did you have another student in the lab peer review your paper for clarity, typos, wrong notation etc.? Send an email to Sandeep (CC'ing both students) with the paper draft. \answerYes{}
  \item Did you make sure all references have the book/conference venue, not just the author and title? \answerNo{}
  \item Did you use the common reference files in the lab GIT, making sure to put our internal papers in ref/SwarmLabPubs.bib and all other papers in ref/external.bib? \answerYes{}
  \item Did you outline your paper and place the DARPA Heilmeier Catechism question answers at the top of the outline? \answerNo{}
\end{enumerate}

% TODOs:
% \begin{enumerate}
%   \item Mathematical definition of cooperative games and convex games in the Appendix. \answerTODO{}
%   \item Add more citations. \answerTODO{}
% \end{enumerate}

\newpage


==> sections/related.tex <==
Data collection from networked robots is related to cloud robotics \cite{goldbergwebsite, kehoe2015survey, kuffner2010cloud, Chinchali2010HarvestNetMV, goldberg2013cloud, chinchali2019RSS, tanwani2019fog, geng2021decentralized, pujol2021fog} and  active learning \cite{Cohn96activelearning, pmlr-v70-gal17a, settles2009active, tong2001active, ActLearn4wireless}. In such prior works, robots either send \textit{all} their data to the cloud
or select samples individually without coordination. 
In contrast, we exploit the fact that networked AVs can coordinate how to sample rare data to achieve a better outcome (i.e., balanced data distribution).

Federated learning (FL) \cite{fl, fedler, XIANJIA2021135, OptSampling4FL, armacki2022personalized, WirelessDSGD, PrivacyAsyncFL, FLSurveyPaper, caldas2018expanding} enables a fleet of mobile devices to train ML models on local private data and only share anonymized gradient updates with the cloud. However, our work is fundamentally different, and even complementary, to standard FL.  First, FL makes the restrictive assumption that each robot has perfectly labeled local data,
which is infeasible for AVs that observe rare, OoD images. Instead, we address a practical scenario where robots run local inference with only an \textit{imperfect} vision model that guides data collection.
Moreover, FL does not statistically sample data but trains on all of it locally, while our approach only uploads a limited set of images to reduce network and data labeling costs. Finally, we assume robots only receive ground-truth labels for the uploaded data in the cloud, which is required for training on rare classes. 

In N-person cooperative games, players join forces to achieve a common goal, whereas, in non-cooperative games, each player plays greedily \cite{Rosen1965Existence, KIM20021219, wang1988theory, driessen2013cooperative, Stuart2001, tijs2003introduction}. 
In convex games, the incentives to join a coalition increase as the coalition size  grows, which is the case in our setting since adding new robots leads to a diverse cloud dataset and, therefore, faster convergence to a target dataset. N-person cooperative concave/convex games have been studied extensively, such as for wireless network resource allocation. However, to the best of our knowledge, ours is the first work to contribute a game-theoretic
formulation for distributed data collection from a fleet of robots.


